JaqalPaw: A Guide to Defining Pulses and Waveforms for Jaqal

One of the many challenges of developing an open user testbed such as QSCOUT is providing an interface that maintains simplicity without compromising expressibility or control. This interface comprises two distinct elements: a quantum assembly language designed for specifying quantum circuits at the gate level, and a low-level counterpart used for describing gates in terms of waveforms that realize specific quantum operations. Jaqal, or "Just another quantum assembly language," is the language used in QSCOUT for gate-level descriptions of quantum circuits. JaqalPaw, or "Jaqal pulses and waveforms," is its pulse-level counterpart. This document concerns the latter, and presents a description of the tools needed for precisely defining the underlying waveforms associated with a gate primitive.

==> PhaseWinding.tex <==
% ['CubicSpline3Tex.py', '5', '(0,120,740,1100,-1100,-740,-120,0)', '-y', 'Phase 0 (deg.)']

    \begin{tikzpicture}
            \pgfplotsset{ 
                scale only axis,
                xmin=-0.5,xmax=7.5,
                %ymin=-1100.5,ymax=1100.5,
                ymin=-0.5,ymax=1210.0,
                every axis plot/.append style={line join=round,line cap=round,clip=false}
            }

            \begin{axis}[
                width=\linewidth,
                xlabel=Time ($\mu$s),
                ylabel=Phase 0 (deg.),
                samples=100,
                xticklabels={0.00,0.71,1.43,2.14,2.86,3.57,4.29,5.00},
                xtick={0.0,1.0,2.0,3.0,4.0,5.0,6.0,7.0}
                ]
    \addplot[draw=black][domain = 0.0:1.0]{90.73171*((x-0.0)/(1.0))^3+-0.00000*((x-0.0)/(1.0))^2+29.26829*((x-0.0)/(1.0))^1+0.00000*((x-0.0)/(1.0))^0};
\addplot[draw=black, forget plot][domain = 1.0:2.0]{46.34146*((x-1.0)/(1.0))^3+272.19512*((x-1.0)/(1.0))^2+301.46341*((x-1.0)/(1.0))^1+120.00000*((x-1.0)/(1.0))^0};
\addplot[draw=black, forget plot][domain = 2.0:3.0]{-1036.09756*((x-2.0)/(1.0))^3+411.21951*((x-2.0)/(1.0))^2+984.87805*((x-2.0)/(1.0))^1+740.00000*((x-2.0)/(1.0))^0};
\addplot[draw=black, forget plot][domain = 3.0:4.0]{1798.04878*((x-3.0)/(1.0))^3+-2697.07317*((x-3.0)/(1.0))^2+-1300.97561*((x-3.0)/(1.0))^1+1100.00000*((x-3.0)/(1.0))^0};
\addplot[draw=black, forget plot][domain = 4.0:5.0]{-1036.09756*((x-4.0)/(1.0))^3+2697.07317*((x-4.0)/(1.0))^2+-1300.97561*((x-4.0)/(1.0))^1+-1100.00000*((x-4.0)/(1.0))^0};
\addplot[draw=black, forget plot][domain = 5.0:6.0]{46.34146*((x-5.0)/(1.0))^3+-411.21951*((x-5.0)/(1.0))^2+984.87805*((x-5.0)/(1.0))^1+-740.00000*((x-5.0)/(1.0))^0};
\addplot[draw=black, forget plot][domain = 6.0:7.0]{90.73171*((x-6.0)/(1.0))^3+-272.19512*((x-6.0)/(1.0))^2+301.46341*((x-6.0)/(1.0))^1+-120.00000*((x-6.0)/(1.0))^0};
        \end{axis}
    \end{tikzpicture}
    


==> __latexindent_temp.tex <==
          sync_mask=0b00,          # synchronize phase for current frequency

==> code/anatomy/sidebyside.jaqal.tex <==
from GateFile.GatePulse usepulses *
register q[8]
G q[2]


==> code/anatomy/sidebyside.py.tex <==
class GatePulse:
    def gate_G(self, qubit):
        return ...


==> code/anatomy/simple_gp_class.py.tex <==
import numpy as np
from qscout.v1.QSCOUTBuiltins import QSCOUTBuiltins

class GatePulse(QSCOUTBuiltins):

    calibrated_amplitude : float = 45.0

    @staticmethod
    def gauss(amp, sigma, num_points):
        x_points = np.linspace(-1.0, 1.0, num_points)
        return amp * np.exp(-x_points**2/2/sigma**2)

    def gate_G(self, qubit, phi):
        scaled_amp = self.calibrated_amplitude * phi / np.pi
        amplitude_envelope = self.gauss(scaled_amp, .3, 7)
        return [PulseData(...)]
        


==> code/frequency_feedback/gpFeedbackEnableCoProp.py.tex <==
def gate_G_coprop(self, qubit):
    return [PulseData(qubit, 1e-6,
                      freq0=200e6,
                      freq1=242e6,
                      amp0=50,
                      amp1=50,
                      fb_enable_mask=0b10)]


==> code/frequency_feedback/gpFeedbackEnableCounterProp.py.tex <==
def gate_G_counterprop(self, qubit):
    return [PulseData(GLOBAL_BEAM, 1e-6,
                      freq0=242e6,
                      amp0=50,
                      fb_enable_mask=0b01),
            PulseData(qubit, 1e-6,
                      freq0=200e6,
                      amp0=50,
                      fb_enable_mask=0b00)]

==> code/pulsedata/gpFrameRotApplyAtEnd.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit, 1e-6,
                      framerot0=10,
                      apply_at_end_mask=1),
            PulseData(qubit, 1e-6),  # NOP
            PulseData(qubit, 1e-6,
                      framerot0=-5,
                      rst_frame_mask=1)]

==> code/pulsedata/gpFrameRotFwdAndInv.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit, 1e-6,
                      framerot0=15,
                      fwd_frame0_mask=0b01,
                      inv_frame0_mask=0b00),
            PulseData(qubit, 1e-6,
                      framerot0=15,
                      fwd_frame0_mask=0b10,
                      inv_frame0_mask=0b10),
            PulseData(qubit, 1e-6,
                      framerot0=15,
                      fwd_frame0_mask=0b11,
                      inv_frame0_mask=0b01)]

==> code/pulsedata/gpFrameRotSingle.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit, 1e-6,
                      framerot0=10)
            for _ in range(3)]

def gate_G(self, qubit):
    return [PulseData(qubit, 3e-6,
                      framerot0=[10,10,10]
                      )]

==> code/pulsedata/gpFrameRotSpline.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit, 1e-6,
                      framerot0=15),
            PulseData(qubit, 3e-6,
                      framerot0=(0,10,-10,-5)),  
            PulseData(qubit, 1e-6)]  # NOP

==> code/pulsedata/gpPiecewise.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit, 2e-6, 
                      amp0=(0,9,41,50)),
            PulseData(qubit, 2e-6, 
                      amp0=50),
            PulseData(qubit, 2e-6, 
                      amp0=(50,0))]



==> code/pulsedata/gpPiecewiseCounter.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit, 2e-6, 
                      amp0=(0,9,41,50)),
            PulseData(qubit, 2e-6, 
                      amp0=50),
            PulseData(qubit, 2e-6, 
                      amp0=(50,0)),
            PulseData(GLOBAL_BEAM, 4.5e-6,
                      amp0=(0,30,20,70)]



==> code/pulsedata/gpSplineDiscreteComb.py.tex <==
def gate_G(self, qubit):
    spline_amps = (10,30,20,50,20,60,30,50)
    discrete_amps = [10,30,20,30,50]
    return [PulseData(qubit, 
                      5e-6, 
                      freq0=200e6,
                      freq1=230e6,
                      amp0=spline_amps,
                      amp1=discrete_amps)]



==> code/pulsedata/gpdiscrete.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit, 
                      5e-6, 
                      freq0=200e6,
                      amp0=[10,30,20,50],
                      phase0=0)]




==> code/pulsedata/gpplain.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit,       # output channel
                      1.25e-6,     # duration (s)
                      freq0=200e6, # frequency (Hz)
                      amp0=50,     # amplitude (arb.)
                      phase0=0)]   # phase (deg.)




==> code/pulsedata/gpsmooth.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit, 
                      5e-6, 
                      freq0=200e6,
                      amp0=(10,30,20,50),
                      phase0=0)]



==> code/pulsedata/gpsquaregapmulti.jaqal.tex <==
G_gap_multi q[2] 4


==> code/pulsedata/gpsquaregapmulti.py.tex <==
def gate_G_gap_multi(self, qubit, loops):
    return [PulseData(qubit, 1.25e-6, amp0=50),
            PulseData(qubit, 0.25e-6)] * loops



==> code/pulsedata/gpsquaregapsep.jaqal.tex <==
loop 4 {
  G q[2]
  gap q[2]
}


==> code/pulsedata/gpsquaregapsep.py.tex <==
def gate_G(self, qubit):
    return [PulseData(qubit, 1.25e-6, amp0=50)]

def gate_gap(self, qubit):
    return [PulseData(qubit, .25e-6)]





==> code/pulsedata/gpsquaregapsingle.jaqal.tex <==
loop 4 {
  G_gap q[2]
}


==> code/pulsedata/gpsquaregapsingle.py.tex <==
def gate_G_gap(self, qubit):
    return [PulseData(qubit, 1.25e-6, amp0=50),
            PulseData(qubit, 0.25e-6)]



==> code/pulsedata/pulsedata.py.tex <==
PulseData(channel,                 # output channel
          dur,                     # total duration to apply parameters (s)
          freq0=0,                 # tone 0 frequency (Hz)
          phase0=0,                # tone 0 phase (deg.)
          amp0=0,                  # tone 0 amplitude (arb.)
          freq1=0,                 # tone 1 frequency (Hz)
          phase1=0,                # tone 1 phase (deg.)
          amp1=0,                  # tone 1 amplitude (arb.)
          framerot0=0,             # frame 0 virtual rotation (deg.)
          framerot1=0,             # frame 1 virtual rotation (deg.)
          # metadata parameters (XXX_mask indicates per-tone settings)
          sync_mask=0b00,          # synchronize phase for current frequency
          enable_mask=0b00,        # toggle the output enable state
          fb_enable_mask=0b00,     # enable frequency correction
          apply_at_end_mask=0b00,  # apply frame rotation at end of pulse
          rst_frame_mask=0b00,     # reset accumulated frame rotation
          fwd_frame0_mask=0b00,    # forward frame 0
          fwd_frame1_mask=0b00,    # forward frame 1
          inv_frame0_mask=0b00,    # invert frame 0 sign
          inv_frame1_mask=0b00,    # invert frame 1 sign 
          waittrig=False)          # wait for external trigger



==> code/synchronization/discretize_frequency_example.py.tex <==
from jaqalpaw.utilities.helper_functions import discretize_frequency

class GatePulse:

    aom_center_frequency: float = 200e6
    effective_qubit_splitting: float = 28.123e6
    motional_mode_frequencies: float = [2.5e6, 
                                        2.42e6, 
                                        2.38e6, 
                                        ...]
    amplitude_scaling: float = [.97,
                                .96,
                                .95,
                                ...]

    def gate_G(self, qubit1, qubit2):
        global_aom_frequency = (self.aom_center_frequency + 
                                self.effective_qubit_splitting)
        individual_aom_frequency = self.aom_center_frequency
        sb_freq = discretize_frequency(motional_mode_frequencies[0])
        qubit_freq = discretize_frequency(global_aom_frequency)
        rsb_freq = qubit_freq - sb_freq
        bsb_freq = qubit_freq + sb_freq

        return [PulseData(GLOBAL_BEAM, 100e-6,
                          freq0=rsb_freq,
                          freq1=bsb_freq,
                          fb_enable_mask=0b11,
                          sync_mask=0b11),
                PulseData(qubit1, 100e-6,
                          freq0=individual_aom_frequency
                          sync_mask=0b01),
                PulseData(qubit1, 100e-6,
                          freq0=individual_aom_frequency
                          sync_mask=0b01),
                          ]


==> figures/synchronization/__latexindent_temp.tex <==
                        xticklabels={$f=f_0$,$f\rightarrow f_1$,$f\rightarrow f_0$,},

==> figures/synchronization/globalSyncAllFreqs.tex <==
\begin{tikzpicture}

	\pgfplotsset{
		scale only axis,
		xmin=0.0,xmax=2.0,
		ymin=-1.1,ymax=1.1,
		every axis plot/.append style={line join=round,line cap=round,clip=false}
	}

	\begin{axis}[
		width=0.5\linewidth,
		xlabel=Time,
		ylabel=Amplitude,
		samples=100,
		xticklabels={,,},
		xtick={0,1,2},
		ytick={-2,2},
		yticklabels={,},
		cycle list name=linestyles*,
	]

		\foreach \i in {10,...,20}{
			\addplot+[domain = 0:2]{sin(\i/4*deg(x))};
		}

	\end{axis}
\end{tikzpicture}



==> potpourri.tex <==
\section{Potpourri}

This section contains specialized details and corner cases.

\subsection{Pulse Collisions}

When running gates in parallel from the Jaqal level such as
\begin{Jaqal}
    < X q[1] | Y q[2] >
\end{Jaqal}
may require additional consideration depending on how the pulses are defined.
Pulses that address the same channel at the same time can collide.
In some cases this may be necessary, for instance when the \li{GLOBAL_BEAM} channel is needed for both operations.
JaqalPaw will allow these cases when the \pd objects on the shared channel(s) are identical.

\subsection{Phase Winding}

Phase inputs, including \li{phase0}, \li{phase1}, \li{frame0}, and \li{frame1}, are generally converted modulo 360$^\circ$ when encoded for hardware.
However, these inputs do support continuous modulation across the phase boundaries.
For splines, the modulus is taken for the zeroth order spline coefficients after the spline has been fit.
\begin{figure}
    \include{PhaseWinding.tex}
\end{figure}

